A Systematic Survey and Critical Review on Evaluating Large Language Models: Challenges, Limitations, and Recommendations

Large Language Models (LLMs) have recently gained significant attention due to their remarkable capabilities in performing diverse tasks across various domains. However, a thorough evaluation of these models is crucial before deploying them in real-world applications to ensure they produce reliable performance. Despite the well-established importance of evaluating LLMs in the community, the complexity of the evaluation process has led to varied evaluation setups, causing inconsistencies in findings and interpretations. To address this, we systematically review the primary challenges and limitations causing these inconsistencies and unreliable evaluations in various steps of LLM evaluation. Based on our critical review, we present our perspectives and recommendations to ensure LLM evaluations are reproducible, reliable, and robust.

==> not_needed/removed_text.tex <==

%To conduct a systematic survey on the challenges and limitations of existing benchmarks, 
%\textit{diverse capabilitiy benchmarks}, and \textit{independent benchmarks}. %We give a brief overview of each benchmark below and show the taxonomy of these benchmarks in Figure \ref{fig:taxonomy}.


%In addition to general reasoning capabilities, the tasks in these benchmarks are applicable to a wide range of domains, such as biomedical \cite{jahan2024comprehensive}, finance \cite{li2023largefinance,guo2023chatgptfinance}, social science \cite{ziems2024cansocialscience}, coding \cite{liu2024yourcode}, information retrieval \cite{zhu2023large} etc. %%SAWSAN: ADD FEW STATEMENTS REGARDING THESE DATASETS



% In addition to that, ethics, bias, toxicity, robustness, and trustworthiness are also important criteria for LLM evaluation \cite{yang2022gluerobustness,wang2023robustness,zhuo2023redteaming,rawte2023surveyhallucination,liu2023mitigatinghallucination,zhu2023promptbench,mcintosh2024inadequacies}. %Thus, the evaluation of LLMs has become an important research area in recent years \cite{laskar-etal-2023-systematic,bang2023multitaskchatgpt,qin2023chatgpt}. 
% % also evaluate LLMs across a set of selected datasets, covering various domains, such as biomedicine \cite{jahan2024comprehensive}, , etc. 

% When examining the literature on language model evaluation, we find various overlapping yet distinct task categorizations that describe model capabilities and behavior. One categorization is the one suggested by \cite{llm_eval_tist} in which tasks used for LLM evaluation can be categorized into: (i) natural language understanding, (ii) natural language generation, (iii) reasoning, (iv) factuality, and (v) multilinguality. These tasks are applicable to a wide range of domains, such as biomedical \cite{jahan2024comprehensive}, finance \cite{li2023largefinance,guo2023chatgptfinance}, social science \cite{ziems2024cansocialscience}, coding \cite{liu2024yourcode}, information retrieval \cite{zhu2023large} etc. 
% In addition to that, ethics, bias, toxicity, robustness, and trustworthiness are also important criteria for LLM evaluation \cite{yang2022gluerobustness,wang2023robustness,zhuo2023redteaming,rawte2023surveyhallucination,liu2023mitigatinghallucination,zhu2023promptbench,mcintosh2024inadequacies}. %Thus, the evaluation of LLMs has become an important research area in recent years \cite{laskar-etal-2023-systematic,bang2023multitaskchatgpt,qin2023chatgpt}. 
% % also evaluate LLMs across a set of selected datasets, covering various domains, such as biomedicine \cite{jahan2024comprehensive}, , etc. 

%The tasks \cite{llm_eval_tist} used for LLM evaluation can be categorized into: (i) natural language understanding, (ii) natural language generation, (iii) reasoning, (iv) factuality, and (v) multilinguality. These tasks are applicable to a wide range of domains, such as biomedical \cite{jahan2024comprehensive}, finance \cite{li2023largefinance,guo2023chatgptfinance}, social science \cite{ziems2024cansocialscience}, coding \cite{liu2024yourcode}, information retrieval \cite{zhu2023large} etc. In addition to that, ethics, bias, toxicity, robustness, and trustworthiness are also important criteria for LLM evaluation \cite{yang2022gluerobustness,wang2023robustness,zhuo2023redteaming,rawte2023surveyhallucination,liu2023mitigatinghallucination,zhu2023promptbench,mcintosh2024inadequacies}. Thus, the evaluation of LLMs has become an important research area in recent years \cite{laskar-etal-2023-systematic,bang2023multitaskchatgpt,qin2023chatgpt}. % also evaluate LLMs across a set of selected datasets, covering various domains, such as biomedicine \cite{jahan2024comprehensive}, , etc. 



%  To benchmark the performance of LLMs, researchers typically evaluate them using a set of common datasets. %Previous studies have been active in this area, introducing various benchmarking datasets that mostly focus on multiple-choice question answering.  
% By common benchmarks, we refer to those datasets that are commonly used by the authors when they release an LLM to evaluate its general capabilities.
% One of the most common benchmarks in this regard is the MMLU benchmark \cite{hendrycks2020measuring}, covering various subjects to assess LLMs overall knowledge and reasoning capabilities \cite{hendrycks2020measuring}. %evaluating models on their ability to select the correct answer from given options. 


% The other common benchmarks mainly focus on evaluating the commonsense reasoning capabilities of LLMs, such as HellaSwag \cite{zellers2019hellaswag}, PIQA \cite{bisk2020piqa}, SIQA, \cite{sap2019siqa}, WinoGrande \cite{sakaguchi2021winogrande}, OpenBookQA \cite{mihaylov2018openbookqa}, ARC \cite{clark2018thinkarq}, etc. In addition, the TruthfulQA \cite{lin2021truthfulqa} dataset is used to measure the truthfulness of an LLM.  Regarding coding capability evaluation, the HumanEval \cite{chen2021evaluating} and the MBPP \cite{austin2021program} are two common coding benchmarks.   % In addition, there are several other challeng  BigBench-Hard \cite{suzgun2022challengingbigbench}. 

%With LLMs already achieving impressive performance on these benchmarks, more challenging versions have been released, such as MMLU-Pro \cite{wang2024mmlupro}, GSM-1K \cite{zhang2024carefulgsm1k}, and BigBench-Hard \cite{suzgun2022challengingbigbench}. Effectively answering multiple-choice questions requires a multifaceted approach. Models must understand the question's objective, analyze each option, eliminate incorrect choices, and determine the best answer, similar to the cognitive process humans use.

%%SAWSAN: TALK ABOUT OTHER TYPES OF BENCHMARKING DATASETS LIKE GENERATION , CLASSIFICATION, ... ETC. 
%GSM-8K \cite{cobbe2021traininggsm8k}, HellaSwag \cite{zellers2019hellaswag}, TruthfulQA \cite{lin2021truthfulqa}, PIQA \cite{bisk2020piqa}, SIQA \cite{sap2019siqa}, OpenBookQA \cite{mihaylov2018openbookqa}, ARC \cite{clark2018thinkarq}, WinoGrande \cite{sakaguchi2021winogrande} etc. 



% Multiple-choice questions sourced from diverse fields of knowledge—ranging from mathematics to US history, computer science, and law—underscore the breadth of domains these evaluations encompass. These assessments function as tests for evaluating language understanding, probing both single-step and multi-step reasoning abilities. Successfully answering these questions often necessitates not just linguistic prowess but also a grasp of worldly knowledge and effective problem-solving skills.



% \paragraph{General Capabilities Benchmarks:} To evaluate the capabilities and limitations of LLMs, LLMs are usually evaluated across a set of common datasets, such as MMLU \cite{hendrycks2020measuring}, GSM-8K \cite{cobbe2021traininggsm8k}, HellaSwag \cite{zellers2019hellaswag}, TruthfulQA \cite{lin2021truthfulqa}, PIQA \cite{bisk2020piqa}, SIQA \cite{sap2019siqa}, OpenBookQA \cite{mihaylov2018openbookqa}, ARC \cite{clark2018thinkarq}, WinoGrande \cite{sakaguchi2021winogrande} etc. Among these benchmark datasets, the MMLU (Massive Multitask Language Understanding) benchmark \cite{hendrycks2020measuring} is widely used. This benchmark consists of multiple tasks and domains to assess the language comprehension and reasoning capabilities of LLMs. Another benchmark close to MMLU is BigBench \cite{srivastava2022beyond}. With LLMs already achieving impressive performance in these benchmarks, to make them more challenging, some new versions of these benchmarks are released, such as MMLU-Pro \cite{wang2024mmlupro}, GSM-1K \cite{zhang2024carefulgsm1k}, BigBench-Hard \cite{suzgun2022challengingbigbench}, etc. Meanwhile, due to the importance of comprehensive evaluation of LLMs across a wide range of scenarios, some new benchmarks like HELM \cite{liang2022holistic}, PromptBench \cite{zhu2023promptbench}, OpenLLM\footnote{\url{https://huggingface.co/spaces/HuggingFaceH4/open_llm_leaderboard}} etc. have been introduced recently. These benchmarks consist of both the existing benchmarks (e.g., Big-Bench, MMLU, etc.) alongside various existing task-specific datasets. 


% \paragraph{Specialized Benchmarks:}
%There are also specialized benchmarks that measure specific capabilities of LLMs, such as whether LLMs can engage in conversations. %retrieve relevant information from knowledge bases, and 
%as well as investigate their capability to understand both images and texts, For evaluating the models' ability to follow conversations smoothly and interact properly with users, %several benchmarks have been introduced including Chatbot Arena \cite{zheng2024judging} which assesses LLMs through user engagement and voting and 
%In this regard, benchmarks like MT-Bench \cite{zheng2024judging} have been introduced to assess LLMs using questions that simulate real-world scenarios. 


%Another essential capability that are useful in deploying LLMs in real-time applications provided several advantages over pre-trained or fine-tuned LLMs and is the appropriate retrieval for relevant texts, known as Retrieval Augmented Generation (RAG) \cite{lewis2020retrieval, gao2023retrieval}. Hence, many benchmarks have been introduced recently to assess the LLMs capabilites in this regard, such as RGB \cite{chen2024benchmarking}, RECALL \cite{ liu2023recall}, MIRAGE \cite{xiong2024benchmarking}, MultiHop-RAG \cite{tang2024multihop}, MedExpQA \cite{alonso2024medexpqa}, CRAG,\footnote{(\url{www.aicrowd.com})} CRUD \cite{lyu2024crud}. 


% such as MME~\cite{fu2023mme}, MM-Vet~\cite{yu2023mm}, MMBench~\cite{liu2023mmbench}, Seed-Bench~\cite{li2023seed,li2023seed0}, LLaVA-QA90~\cite{liu2024visual}, and BLINK~\cite{fu2024blink}, which assess tasks ranging from basic recognition to high-level visual understanding. Other benchmarks, like ScienceQA~\cite{lu2022learn}, MMMU~\cite{yue2023mmmu}, HallusionBench~\cite{guan2023hallusionbench}, POPE~\cite{li2023evaluating}, VALOR-BENCH~\cite{qiu2024valor}, MathVista~\cite{lu2023mathvista}, and MMStar~\cite{chen2024we}. 

%Recently, new benchmarks have been introduced to measure specific granular understanding capabilities of LLMs. For instance, the RewardBench \cite{lambert2024rewardbench} benchmark is introduced for the evaluation of reward models. More recently, \citet{xia2024fofo} introduced the FOFO benchmark that emphasized the necessity of evaluating language models' ability to adhere to the requested format in prompts across different domains, distinguishing this from content-following format (i.e., a model may generate reasonable content but not in the exact requested format). This development is motivated by the recognition that general benchmarks assess a model's overall comprehension and instruction-following abilities but do not highlight the fine-grained differences that could make one model superior to another. % In this regard, . %Consequently, the authors introduced FOFO, a benchmark designed to assess language models' capabilities in following complex and domain-specific formats. Their investigation revealed that closed-source LLMs are more proficient at adhering to specified formats and that model behavior varies across domains. 


% There are also specialized benchmarks that measure specific capabilities of LLMs, such as the MT-Bench \cite{zheng2024judging}) benchmark to evaluate whether LLMs can properly engage in conversations,  the RewardBench \cite{lambert2024rewardbench} benchmark to evaluate the reward models, the FOFO benchmark to evaluate language models' ability to adhere to the requested format in prompts across different domains \citet{xia2024fofo}. 
% Another interesting capability of recently proposed LLMs~\cite{zhu2023minigpt, liu2024visual, liu2023improved, dai2024instructblip, zhang2023internlm, ye2023mplug,luo2024cheap, bai2023qwen,chen2023sharegpt4v} is their ability to understand both language and vision which is originated from the CLIP~\cite{radford2021learning} technology. This has led to the development of many multi-modal benchmarks \cite{fu2023mme,yu2023mm,liu2023mmbench,li2023seed,li2023seed0,liu2024visual,fu2024blink,lu2022learn,guan2023hallusionbench,li2023evaluating,qiu2024valor,chen2024we}. These benchmarks study the multimodal capabilities of LLMs across various domains, such as math and reasoning ~\cite{yue2023mmmu,lu2023mathvista}, science diagrams \cite{kembhavi2016diagram}, chart understanding and reasoning \cite{masry2022chartqa}, document understanding \cite{mathew2021docvqa}.
% introduced  that emphasized the necessity of evaluating language models' ability to adhere to the requested format in prompts across different domains, distinguishing this from content-following format (i.e., a model may generate reasonable content but not in the exact requested format). This development is motivated by the recognition that general benchmarks assess a model's overall comprehension and instruction-following abilities but do not highlight the fine-grained differences that could make one model superior to another.

%\paragraph{Diverse Capability Benchmarks (General and Specialized):}

 

% While there are several common benchmarks (both general and specific benchmarks) that are widely used by researchers, all the variety of tasks are not covered in existing benchmarks. Thus, researchers independently evaluated LLMs across various datasets and tasks. In addition to general evaluation across various NLP datasets and tasks \cite{laskar-etal-2023-systematic,bang2023multitaskchatgpt,qin2023chatgpt, kocon2023chatgptjackofalltrades}, there are also specific, focused independent benchmarks, such as biomedical \cite{jahan2024comprehensive}, finance \cite{li2023largefinance,guo2023chatgptfinance}, social science \cite{ziems2024cansocialscience}, coding \cite{liu2024yourcode}, information retrieval \cite{zhu2023large} etc. In addition to that, ethics, bias, toxicity, robustness, and trustworthiness are also independently evaluated by researchers across various datasets \cite{yang2022gluerobustness,wang2023robustness,zhuo2023redteaming,rawte2023surveyhallucination,liu2023mitigatinghallucination,mcintosh2024inadequacies}. 

\if{false}
\begin{figure*}[t!]
    \centering
    \begin{tikzpicture}[
        sibling distance=20mm,
        level distance=20mm,
        edge from parent/.style={draw,-latex},
        every node/.style={font=\scriptsize,align=left,text width=35mm}
    ]
    
    \node [draw, rounded corners, fill=orange!10] (A) {%Common
\textbf{Evaluation Benchmarks}}
        child {node [draw, rounded corners, fill=yellow!20] {
            1. \textbf{General Evaluation}  \\
             2. \textbf{Specific Evaluation}  \\
            3. \textbf{Diverse Evaluation} \\
            4. \textbf{Independent Evaluation} \\ 
        }};
    
    \node [draw, rounded corners, fill=orange!10, right=of A] (B) {\textbf{Evaluation Settings}} %for General Capabilities}
        child {node [draw, rounded corners, fill=yellow!20] {
            1.\textbf{ Prompt Design} %Zero-shot, Few-shot, Chain-of-Thought, etc.
            \\
            2. \textbf{Model Selection} 
            %Closed-Source Models (GPT, Gemini, Claude, etc.) Open-Source models (LLaMA, Mistral, Qwen, Phi, Gemma, etc.) 
            \\
            3. \textbf{Parameter Settings} %topK, topP, Temperature, max input and output tokens, etc. 
            \\
            4. \textbf{Parsing Script Design} %For discriminative tasks. 
            \\
        }};
      
           % 7. MBPP \cite{austin2021program} \\


            
    \node [draw, rounded corners, fill=orange!10, right=of B] (C) {\textbf{Evaluation Methodology}}
        child {node [draw, rounded corners, fill=yellow!20] {
            1. \textbf{Evaluation Approach:} \\ (i) Automatic Evaluation \\ \\ (ii) Human Evaluation \\ (iii) Hybrid Evaluation \\ (iv) LLMs as Evaluators \\ 
            2. \textbf{Evaluation Metrics:} \\ (i) For Language Modeling \\
           (ii) For Downstream Tasks \\
        }};

    
  %  \node [draw, rounded corners, fill=orange!10, right=of C] (D) %{Evaluation Metrics}
   %     child {node [draw, rounded corners, fill=yellow!20] {
   %         1. Evaluating for \\ Language Modeling: \\
   %         2. Evaluating on \\ Downstream Tasks: \\
 %       }};
    \end{tikzpicture}
    \caption{Taxonomy of LLM Evaluation. See Figure \ref{fig:taxonomy} for a detailed taxonomy of evaluation benchmarks.}
    \label{fig:taxonomy_of_evaluation}
\end{figure*}
\fi

%Previous studies have proposed various task taxonomies to better guide researchers in selecting appropriate benchmarking datasets for evaluating language models. There are various overlapping yet distinct task categorizations that describe model capabilities and behaviors \cite{llm_eval_tist}. For instance, \citet{llm_eval_tist} suggested to categorize tasks into: \textit{natural language understanding}, \textit{natural language generation}, \textit{reasoning}, \textit{factuality}, and \textit{multilinguality}. Whereas \cite{guo2023evaluating} categorized LLM evaluation into the groups: \textit{knowledge and capability evaluation}, \textit{alignment evaluation} and \textit{safety evaluation}. 

 %While this may happen due to the absence of details regarding the construction of prompts, as well as the unavailability of LLM output parsing scripts. 

\fi

%To investigate the above concerns, in this paper, we conduct a thorough review of the existing literature and benchmarks to validate their effectiveness for LLM evaluation, alongside validating the methodology used for the evaluation of LLMs, as well as the validity of existing metrics used for LLM evaluation. The following sections of this paper are organized as follows: In Section 3, we review the reliability of existing benchmarks used for LLM Evaluation. Then in Section 4, we validate the methodology used for LLM Evaluation. Afterward, in Section 5, we review the effectiveness of existing metrics used for LLM evaluation. In Section 6, we provide an opinion piece on the evaluation of LLMs based on our comprehensive review %to validate the existing evaluation of LLMs 
%alongside suggesting the future direction for LLM evaluation. Finally, in Section 7, we provide our concluding remarks.
% \if{false}
% When examining the literature on language model evaluation, we find various task categorizations that describe the capabilities and behavior of intelligent models. These categorizations often overlap but also diverge in certain aspects. For example, \citet{llm_eval_tist} divided tasks into natural language processing, robustness, ethics, biases and trustworthiness, social sciences, natural sciences and engineering, medical applications, agent applications, and other applications.

% Evaluating language models is crucial yet complex. Each categorization allows for a deeper exploration of nuanced capabilities, which is essential when selecting the most suitable model from a diverse pool of options.

% Different benchmarking datasets have been created, each tailored to address specific capabilities considered important for particular purposes, whether they are generalized or specialized.


% %\paragraph{Multiple-choice Questions:}



%These tasks are applicable to a wide range of domains, such as biomedical \cite{jahan2024comprehensive}, finance \cite{li2023largefinance,guo2023chatgptfinance}, social science \cite{ziems2024cansocialscience}, etc. Furthermore, various research papers \cite{laskar-etal-2023-systematic,bang2023multitaskchatgpt,qin2023chatgpt} also evaluate LLMs across a set of selected datasets, covering various domains, such as biomedicine \cite{jahan2024comprehensive}, coding \cite{liu2024yourcode,roziere2023code}, information retrieval \cite{zhu2023large}, etc. 

%\subsubsection{Leaderboard}

%Due to the importance of comprehensive evaluation of LLMs across a wide range of scenarios, some new benchmarks like HELM \cite{liang2022holistic}, PromptBench \cite{zhu2023promptbench}, OpenLLM\footnote{\url{https://huggingface.co/spaces/HuggingFaceH4/open_llm_leaderboard}} etc. have been introduced, These benchmarks consist of both the existing benchmarks (e.g., Big-Bench, MMLU, etc.) alongside various existing task-specific datasets.

%In addition to these general NLP benchmarks, there are also some specific, focused benchmarks, such as the Chatbot Arena \cite{zheng2024judging}, which is used to assess chat-focused LLMs through user engagement and voting, while the recently proposed MT-Bench \cite{zheng2024judging} focuses on evaluating LLMs in multi-turn dialogues, using comprehensive questions that simulate real-world scenarios. 

%While prior work \cite{llm_eval_tist,guo2023evaluating} related to LLM evaluation mostly focused on the following aspects: \textit{what to evaluate}, \textit{where to evaluate}, and \textit{how to evaluate}, they did not study several limitations in existing LLM evaluation datasets and benchmarks, the possibility of data contamination and lack of generalizability, as well as whether the findings from these evaluations are reproducible and consistent, and whether various datasets and benchmarks used for LLM evaluation make sense now. Below, we discuss these concerns:



%\fi

%\item \textbf{Review Existing benchmarks:  General domain benchmarks [Tahmid, Sawsan], Multi-Modal [Amran, Tahmid], RAG: [Mizan, Tahmid].}
%luation process of generative models, it is crucial to identify three key components alongside the language model under examination:  evaluation benchmarks, evaluation methodology, and evaluation metrics. Each of these components presents its own set of challenges, and their interplay can introduce further complexities that must be addressed, as we will elaborate on in Section \ref{}.
%\section{Background} 


% To investigate the above concerns, in this paper, we present a comprehensive survey to validate the evaluation of Large Language Models. Based on our survey, we provide an opinion piece on the following research questions:


% \begin{itemize}
%     \item \texttt{Validating the reliability of existing benchmarks used for LLM Evaluation.} %\textit{This includes studying the possibility of data contamination in existing benchmarks, and whether the performance of LLMs in existing benchmarks reflects their true capabilities to solve real-world problems.}
%     \item \texttt{Validating the existing LLM evaluation methodology.} %\textit{This includes studying the effect of parsing scripts to parse LLM-generated responses, and the reliability of using LLMs as evaluators, as well as their potential biases as evaluators.}
%     \item \texttt{Validating the effectiveness of existing evaluation metric used for LLM evaluation.}  %\textit{This includes whether existing evaluation metrics, such as perplexity, or ROUGE, are reliable to evaluate LLM's capabilities and limitations.}
% \end{itemize}

%The degree of complexity involved in evaluating a language model can vary significantly depending on the evaluation's objectives. For instance, testing may focus on the model's ability to perform specific, pre-defined tasks or on its overall effectiveness as a general-purpose language model. The evaluation process becomes even more intricate when considering additional factors, such as the model's ability to quickly adapt to new tasks with minimal effort.

\fi


% \begin{itemize}
%     \item \texttt{Validating the reliability of existing benchmarks used for LLM Evaluation.} %\textit{This includes studying the possibility of data contamination in existing benchmarks, and whether the performance of LLMs in existing benchmarks reflects their true capabilities to solve real-world problems.}
%     \item \texttt{Validating the existing LLM evaluation methodology.} %\textit{This includes studying the effect of parsing scripts to parse LLM-generated responses, and the reliability of using LLMs as evaluators, as well as their potential biases as evaluators.}
%     \item \texttt{Validating the effectiveness of existing evaluation metric used for LLM evaluation.}  %\textit{This includes whether existing evaluation metrics, such as perplexity, or ROUGE, are reliable to evaluate LLM's capabilities and limitations.}
% \end{itemize}




%More specifically, our major contributions are summarized below: 

%\begin{itemize}
  %  \item We first present a comprehensive survey framework that critically studies the full pipeline of LLM evaluation in a structured way to identify the gaps in existing evaluation of LLMs %. Our survey unveils the limitations of existing evaluation approaches 
  %  that effects \textit{reproducibility}, \textit{reliability}, and \textit{robustness} in every step of LLM evaluation [Section 3].  % present a principled guideline on how to tackle them. 
 %   \item Based on our comprehensive survey, we offer a principled guideline %to address existing limitations 
  %  to ensure 
 %   \textbf{reproducibility}, \textbf{reliability}, and \textbf{robustness} of LLM evaluation which is crucial for credible and comparable evaluations [Section 4]. % Based on our findings, we offer an informed perspective 
%on several key research questions 
%in Section \ref{opinion}.  
%\end{itemize}




%\begin{itemize}
 %   \item In order to develop a proper standardization of LLM evaluation, we present a comprehensive survey framework that studies the full pipeline of LLM evaluation in a structured way, unveils the limitations of existing evaluation approaches in every level in the pipeline such as benchmarks, methodologies, and metrics and present a principled guideline on how to tackle them. 
   % \item 
%\end{itemize}

%an informative perspective on the future evaluations of LLMs to ensure a more structured framework for  
%assessing model performance, which is crucial for credible and comparable evaluations. We systematically review the existing evaluations of LLMs 
%to assess the challenges and limitations 
%that emerge from different evaluation setups, %the selection of the right evaluation benchmarks, and the choice of the appropriate evaluation methodology and metric. 
%in the existing evaluations of LLMs




% highlighting the need for stricter and more open evaluation practices to %prevent biases and 
% ensure fairness.


% While some work recently attempted to discuss certain challenges related to the evaluation of LLMs \cite{biderman2024lessons,balloccu2024leak}, 
%  a comprehensive study covering diverse aspects and challenges in evaluating LLMs by combining them into a unified framework remains missing. For instance, \citet{biderman2024lessons} have provided several practical guidelines for evaluation by focusing only on the reproducibility problem and subsequently proposed an open-source evaluation package to standardize the process to enhance reproducibility.  %\citet{llm_eval_tist} have discussed the evaluation process from three dimensions: \textit{what}, \textit{where}, and \textit{how} to evaluate, as crucial components in the evaluation process. 
% Meanwhile, \citet{balloccu2024leak} studied issues related to data contamination and evaluation malpractices in closed-source LLMs, highlighting the need for stricter and more open evaluation practices to %prevent biases and 
% ensure fairness.

%%%%%%% Intro polished above %%%%%%%


% where variations in evaluation settings, data contamination, and various biases can impede reliable, reproducible, and robust evaluations significantly. 



% and developing a principled way of LLM evaluations specifically protocols on selecting evaluation benchmarks, methodologies, and metrics remains an open challenge. 

  % \cite{liang2022holistic, zhu2023promptbench, laskar-etal-2023-systematic, bang2023multitaskchatgpt, qin2023chatgpt, zheng2024judging, llm_eval_tist}, 



% Several 


% numerous efforts to establish evaluation methodologies and protocols 


  %Thus, the evaluation of LLMs has become an important research area in recent years \cite{laskar-etal-2023-systematic,bang2023multitaskchatgpt,qin2023chatgpt}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Limitations: benchmarking datasets

%%SAWSAN: should include discussion of previous survey papers - exactly what's in our paper that is not in their paper
% While some work recently attempted to discuss certain challenges related to the evaluation of LLMs \cite{biderman2024lessons,balloccu2024leak}, 
%  a comprehensive study covering diverse aspects and challenges in evaluating LLMs by combining them into a unified framework remains missing. For instance, \citet{biderman2024lessons} have provided several practical guidelines for evaluation by focusing only on the reproducibility problem and subsequently proposed an open-source evaluation package to standardize the process to enhance reproducibility.  %\citet{llm_eval_tist} have discussed the evaluation process from three dimensions: \textit{what}, \textit{where}, and \textit{how} to evaluate, as crucial components in the evaluation process. 
% Meanwhile, \citet{balloccu2024leak} studied issues related to data contamination and evaluation malpractices in closed-source LLMs, highlighting the need for stricter and more open evaluation practices to %prevent biases and 
% ensure fairness.




%However, none of these studies combined the diverse aspects and challenges in evaluating LLMs into a unified framework. %. . .% combined the diverse aspects and challenges in evaluating LLMs into a unified framework. %, making it difficult to address the broad spectrum of challenges. % to address the broad spectrum of challenges 

%Some studies have discussed such challenges and subsequently proposed evaluation packages as an attempt to help improving the evaluation process. For instance, \citet{biderman2024lessons} have provided several practical guidelines for evaluation concerning reproducibility and subsequently proposed an open-source evaluation package to standardize the process and enhance reproducibility (e.g., statistically significant testing, sampling). \cite{llm_eval_tist} have discussed the evaluation process from three dimensions: what, where, and how to evaluate, as crucial components in the evaluation process. 

%Several other studies on the evaluation of LLMs have explored various aspects of LLM performance and challenges. Thorough surveys have been provided on evaluation dimensions, ranging from technical performance to societal impacts, emphasizing the need for holistic evaluation platforms \cite{chang2024survey, guo2023evaluating}. There has also been a focus on the practical challenges in the reproducibility and transparency of LLM evaluations, with efforts to provide an open-source library to standardize and improve evaluation processes \cite{biderman2024lessons}. 

 

% In this paper, we offer insights and a practical guide for evaluating generative models, highlighting the limitations of current evaluation practices and providing recommendations to ensure reproducible and reliable assessments. %We examine these limitations from two perspectives: the factors affecting evaluation throughout the generative models' development cycle and the critical decisions made during the evaluation process. 
% To mitigate this gap, this paper aims to bring together these discussions by addressing the underlying inconsistencies and decision-making complexities that emerge from different evaluation setups, the selection of the right evaluation benchmarks, and the choice of the appropriate evaluation methodology and metric. We focus on identifying and addressing the gaps in standardization, reliability, and robustness of evaluations. Our approach provides a more structured framework for  
% assessing model performance, which is crucial for credible and comparable evaluations. We systematically review the existing LLM evaluation settings, benchmarks, methodologies, and metrics 
% to validate the evaluations of LLMs to ensure \textbf{reproducibility}, \textbf{reliability}, and \textbf{robustness} (Section \ref{validation}). Based on our findings, we offer an informed perspective on several key research questions in Section \ref{opinion}. 

%The major contributions of this research are summarized below: 
%\begin{itemize}
%\item {We conduct a systematic survey to validate the evaluation of LLMs, in terms of evaluation benchmarks, evaluation methodologies, and evaluation metrics. }
%    \item {Based on our comprehensive review, we validate the following research questions: Do the existing evaluations of LLMs ensure \textbf{(i) reproducibility}, \textbf{(ii) reliability}, and \textbf{(iii) generalizibility}?} %: How do we choose which abilities to assess, balance performance trade-offs, pick suitable benchmarking data, and decide the depth of evaluation for each ability? 
%    \item {Finally, we provide our opinion piece and recommendation to ensure a fair, rigorous, and reproducible evaluation of LLMs.} % in the future?} 
%\end{itemize}


\if{false}
\section{XX}
For the evaluation of LLMs, usually various publicly available benchmarks are used to evaluate their reasoning capabilities, mathematical and coding abilities, world knowledge of different domains (law, history, computer science, social science, etc.), factual correctness, ethical aspects, potential biases, etc. However, these existing benchmarks may have several limitations. For instance, recently it has been found that the HumanEval dataset \cite{chen2021evaluating}, which is widely used to evaluate the coding ability of LLMs has insufficient test cases for many problems \cite{liu2024yourhumanevalplus}. Thus, a model may bypass the test cases of a given problem in HumanEval without generating the correct code. Meanwhile, in some tasks like summarization, LLM-generated responses are even preferred over gold reference summaries, questioning the reliability of existing summarization datasets used for evaluation \cite{pu2023summarization}.  

In addition, there is a risk of data contamination in the existing benchmarks \cite{ravaut2024much,xu2024benchmarking,balloccu2024leak} since LLMs are pre-trained on a vast amount of text data available on the internet. This may make the existing evaluation unfair if LLMs have already seen the datasets used for benchmarking during the pre-training phase. For instance, it has been found recently that LLMs usually perform better on datasets that were published before their knowledge cut-off date, but underperform on datasets that are published after their release \cite{li2023taskcontamination}. This raises concerns about LLMs being contaminated %with problems in Codeforces
with datasets that were published before their knowledge cut-off date, making it important to \textbf{\textit{validate the reliability of existing benchmarks used for LLM evaluation}}. 



% Recently, instruction-tuning capable LLMs such as ChatGPT have demonstrated impressive performance across a wide range of tasks in zero-shot and few-shot learning scenarios. This helps empower a set of new real-world applications via leveraging LLMs, such as building chatbots, performing tasks like text summarization and machine translation, programming code generation, as well as solving various analytical problems without requiring any task-specific fine-tuning on large annotated datasets. %This impressive performance of LLMs that was scarcely imaginable just a few years ago. 
% However, a rigorous evaluation is needed before utilizing LLMs in the real world to ensure that LLMs do not generate unfaithful, toxic, or harmful content. 

% For the evaluation of LLMs, usually various publicly available benchmarks are used to evaluate their reasoning capabilities, mathematical and coding abilities, world knowledge of different domains (law, history, computer science, social science, etc.), factual correctness, ethical aspects, potential biases, etc. However, these existing benchmarks may have several limitations. For instance, recently it has been found that the HumanEval dataset \cite{chen2021evaluating}, which is widely used to evaluate the coding ability of LLMs has insufficient test cases for many problems \cite{liu2024yourhumanevalplus}. Thus, a model may bypass the test cases of a given problem in HumanEval without generating the correct code. Meanwhile, in some tasks like summarization, LLM-generated responses are even preferred over gold reference summaries, questioning the reliability of existing summarization datasets used for evaluation \cite{pu2023summarization}.  In addition, there is a risk of data contamination in the existing benchmarks \cite{ravaut2024much,xu2024benchmarking} since LLMs are pre-trained on a vast amount of text data available on the internet. This may make the existing evaluation unfair if LLMs have already seen the datasets used for benchmarking during the pre-training phase. For instance, it has been found recently that LLMs usually perform better on datasets that were published before their knowledge cut-off date, but underperform on datasets that are published after their release \cite{li2023taskcontamination}. This raises concerns about LLMs being contaminated %with problems in Codeforces
% with datasets that were published before their knowledge cut-off date. 
% Thus, it is important to \textbf{\textit{validate the reliability of existing benchmarks used for LLM evaluation}}. 


%One such example is that LLMs could solve competitive programming problems in Codeforces that were published before their knowledge cut-off date, but significantly fail to solve problems published after their release. This raises concerns about whether LLMs are already contaminated with problems in Codeforces that were published before their knowledge cut-off date.

Furthermore, LLMs, more specifically the closed-source ones, only generate human-like text responses instead of providing any probability distribution of the generated tokens. Thus, the common way of evaluating model-generated outputs based on the probability distribution in the classification layer is also not applicable to many discriminative tasks \cite{laskar-etal-2023-systematic}. Since LLMs may sometimes generate additional text in their response in addition to the required output, many researchers write parsing scripts to extract the required output from the LLM-generated response \cite{laskar-etal-2023-systematic,jahan2024comprehensive}. However, the parsing scripts used in various evaluation benchmarks are not consistent \cite{qin2023chatgpt,bang2023multitaskchatgpt,laskar-etal-2023-systematic}, as they differ depending on the authors of the parsing scripts. Meanwhile, since writing such parsing scripts can be very difficult for many complex tasks \cite{jahan2024comprehensive}, researchers are also using LLMs as the judge to evaluate the responses generated by different LLMs \cite{zheng2024judging}. However, using LLMs as judges may also create biases, such as position bias \cite{hou2024llmpositionbias}, while some LLMs may prefer the responses that are generated in their own writing styles \cite{zheng2024judging}. Therefore, it is also important to \textbf{\textit{validate the methodology of LLM evaluation in existing benchmarks}} in terms of various scenarios, such as the reliability of using LLMs as evaluators, the effectiveness of using parsing scripts to parse the required output from LLM-generated responses, etc. 

Moreover, due to the increasing interest in deploying LLMs for real-world usage \cite{laskar2023building,fu2024tiny}, investigating whether existing metrics used for the evaluation of LLMs reflect the true capabilities and limitations of LLMs. % to solve real-world problems. Meanwhile, 
For instance, to deploy LLMs in the real world, while several optimization techniques \cite{frantar2022optq,wan2023efficient,bai2024beyondefficient} are usually applied to LLMs, these optimized LLMs are usually evaluated only based on the perplexity metric on certain benchmarks, without having any extensive evaluation on the targeted downstream tasks. Regarding evaluation metrics, it has been recently found that humans prefer LLM-generated summaries over existing ROUGE metric-based state-of-the-art model-generated summaries \cite{laskar-etal-2023-systematic}. Thus, it is also required to \textbf{\textit{validate the effectiveness of using certain evaluation metrics}} to study whether the performance of LLMs on a particular benchmark in terms of a specific evaluation metric provides true insights into LLM's capabilities and limitations in a particular downstream task, as well as how the results in existing benchmarks align with human ratings.


\if{false}
\section{Literature Review} 

The release of ChatGPT has drawn a lot of interest among researchers to evaluate its capabilities and limitations across benchmark datasets and tasks. In addition to evaluating ChatGPT and other LLMs in existing datasets and tasks, numerous new benchmarks are also recently proposed for the evaluation of LLMs across various domains and modalities. While the early evaluation of ChatGPT required researchers to give task-specific prompts as input to the web interface of ChatGPT, the release of its API has made it possible for researchers to conduct large-scale evaluations. The success of ChatGPT has also led to the introduction of more powerful LLMs, such as Claude, Gemini, LLaMA, etc. 

Although except LLaMA, the above mentioned LLMs are closed-source and only available to use via their respective API or web interface, the release of LLaMA as an open-source LLM has led to a significant increase in the development of more open-source LLMs, such as Mistral, Falcon, Phi, etc. While the original LLaMA model was only available for research purposes, the release of LLaMA-2 has also inspired researchers and practitioners in the industry to develop LLM-based applications due to its availability for commercial purposes. Thus, with this availability of thousands of LLMs, it has become very important to identify the capabilities and limitations of these LLMs across diverse datasets, domains, and tasks. 

Note that LLMs are pre-trained over vast amounts of internet data, and information related to the source of their pre-training corpora is also not generally available. Thus, it has become very challenging to ensure a fair evaluation of these LLMs in existing benchmarks due to the risk of data contamination, i.e., the presence of data from existing benchmarks in LLMs pre-training data. Since the closed-source LLMs are only accessible via their respective APIs, any updates to these closed-source LLMs may make the evaluation of their older versions obsolete. Thus, it is important to evaluate any new updates of these closed-source LLMs to investigate their capabilities and limitations, alongside ensuring reproducibility and replicability of the experiments. Moreover, there can be several discrepancies in terms of the methodology used for the evaluation of LLMs in various benchmarks as well as the prior work. For instance, some benchmarks may rely on other LLMs to evaluate the LLM-generated response, whereas some benchmarks may rely on humans to rate the responses generated by LLMs. In addition, findings in various LLM-based evaluation work may not be consistent as well (e.g., the performance of GPT-4 in the HumanEval benchmark is found to be different in various studies). Meanwhile, evaluation metrics like ROUGE which is widely used to evaluate various tasks may not be reliable anymore since recent studies show that humans tend to prefer LLM-generated responses over non-LLM-based state-of-the-art models in terms of ROUGE metric for tasks like summarization, even though the ROUGE scores for LLM-generated responses are significantly lower. 
 %Below, we briefly discuss each component.% 
%(also see Figure \ref{fig:taxonomy_of_evaluation}). 

%We present a comprehensive survey framework that systematically examines the entire pipeline of LLM evaluation in Section \ref{background}. Our study reveals several inconsistencies and decision-making complexities at every level of the pipeline that affects the reproducibility, reliability, and robustness of evaluation (see Section \ref{validation}). Based on findings, we offer a principled guideline in Section \ref{opinion} to mitigate the existing  limitations in LLM evaluation. 



% Large Language Models (LLMs) have drawn a lot of attention recently due to their impressive capabilities to solve a wide range of tasks across various domains. This has led to a rapid advancement in the development of LLMs. Nonetheless, a rigorous and comprehensive evaluation of these LLMs is needed before utilizing them in the real world to ensure that LLMs do not generate unfaithful or harmful content. %While LLMs are usually evaluated on traditional benchmarks, such as MMLU, PIQA, SIQA, HumanEval, and Elo, certain limitations in these common benchmarks may fail to capture the true capabilities and limitations of LLMs. 
% In this regard, this paper provides an opinion piece based on a comprehensive review of the evaluation of LLMs, % across general and domain-specific scenarios, 
% considering the significance of reliability, reproducibility, and robustness in model assessment. % and the impact of low-resource contexts. 
% Furthermore, we study whether there is a correlation in terms of evaluating LLMs based on certain evaluation metrics in comparison to their % real-world 
% application-specific suitability. % in terms of speed, memory, and accuracy for different LLMs. 
% We also investigate the reliability of using parsing scripts to evaluate LLM-generated responses, as well as the potential biases of using LLMs as evaluators. Lastly, we explore the future directions in LLM benchmarking, emphasizing the need for reliable evaluation metrics and methodology, data contamination analysis, and real-world applicability.

%This leads to the rapid development of real-world applications powered by LLMs. %alongside expanding to include multi-modal processing \cite{openai2023gpt4} and advanced reasoning.

% With the advancements and broad applicability of LLMs comes the responsibility of rigorously and responsibly evaluating. 


% With the advancements and broad applicability of LLMs, proper evaluation becomes crucial for assessing their performance, improving capabilities, ensuring fairness, safety, and robustness, and most importantly, facilitating their informed integration into real-life applications. Therefore, it is essential to understand how effective are our existing forms of LLM evaluation, their bottlenecks or challenges and how to overcome those in order to develop a proper standardization of LLM evaluation. To address, in this paper, we present a comprehensive survey framework that studies the full pipeline of LLM evaluation in an structured way, unveils the limitations of existing evaluation approaches in every level in the pipeline such as benchmarks, methodologies, and metrics and present a principled guideline on how to tackle them. 

%\begin{figure}[t!]
%	\centering
%		\includegraphics[width=\linewidth]{figs/reproducibility_fairness.png}
%\vspace{-3mm}
%	\caption{\small{Reproducibility and Fairness Concerns.}}
% \vspace{-3mm}
% \label{fig:rep_fair}
%\end{figure}

%While 

 %\citet{balloccu2024leak} recently investigated data contamination and evaluation malpractices in LLM evaluation, their study is only limited to the assessment of closed-source LLMs, similar to \citet{mao2023gpteval}, overlooking the whole pipeline of LLM evaluation. 



 
 %More recently, \citet{biderman2024lessons} proposed the \textit{Language Model Evaluation Harness} library for the evaluation of LLMs. However, their work is more focused to address the certain reproducibility problems in existing LLM evaluation, without any comprehensive discussions on how aspects like reliability and robustness may impact LLM evaluation, and how to address them. Hence, despite having immense significance, existing LLM evaluation studies often focus on individual aspects in a scattered manner, resulting in findings that are sparsely useful. 

%\rizwan{Also, the challenges seem not that tough just combining prev works as appears reading the context, and the story seems still incomplete. Why this task we are targeting is challenging?}

%% evaluation settings. % inconsistencies and decision-making complexities that emerge from different evaluation setups, the selection of the right evaluation benchmarks, and the choice of the appropriate evaluation methodology and metric. 



%hybrid evaluation methodology%that combines automatic and human evaluation
%, followed by the %widely used 

 % leveraging human validations. %Regarding human evaluation of LLM-generated responses, the Elo benchmark is introduced which is widely used to evaluate LLM-generated responses via leveraging humans. Below, we describe the Elo benchmark:

%\begin{itemize}

%\item 
%\textbf{How does the Elo benchmark work? What does it take to ensure the Elo benchmark is robustly evaluating LLMs (what are the indicators)? [Zarzis, Sawsan, Rizwan]}






%\textbf{Suggested resources (not limited to): }
%\begin{enumerate}
%    \item \url{https://arxiv.org/pdf/2311.17295}
%\end{enumerate}
%\end{itemize}

\fi
\if{false}

\paragraph{Automatic Evaluation:} 
\label{evaluation_approach}

To provide a high-level overview, automatic evaluation for LLMs can be divided into the following categories:

\textbf{\textit{Language Modeling:}} Perplexity \cite{jelinek1977perplexity} is widely used to study the performance of auto-regressive language models. It measures how confidently a model predicts the next word in a sequence, with the assumption that lower perplexity indicates better performance. Hence, perplexity has been historically used to assess the language model's capability to generate a coherent language and is also useful to quickly compare different models or checkpoints.

% Perplexity reflects the model's confidence in its predictions: lower perplexity signifies higher confidence. 



% parsing scripts are usually not required \cite{laskar-etal-2023-systematic,jahan2024comprehensive} and so the full response generated by LLMs are compared against the gold reference. In this regard, \textit{ROUGE} \cite{lin2004rouge} and \textit{BLEU} \cite{bleu} which are based on n-gram word matching are widely used. Meanwhile, various contextualized similarity-based metrics (e.g., \textit{BERTScore} \cite{zhang2019bertscore}) are also utilized that do not depend on word-based similarity measures. In addition, qualitative evaluation based on \textit{fluency}, \textit{coherence}, \textit{informativeness}, and \textit{factual correctness} are also used \cite{fu2024tiny}. Since LLM-generated responses are usually descriptive, fluent, and also coherent, the hallucination problems \cite{huang2023survey} in LLMs make the qualitative evaluation of \textit{factual correctness} more important. 

% The evaluation metrics vary depending on the task. Tasks that depend on metrics like string matching (e.g., ROUGE \cite{lin2004rouge}) or contextual similarity (e.g., BERTScore \cite{zhang2019bertscore}), do not require the parsing of LLM-generated responses and so a direct comparison between the full response generated by LLMs against the gold reference can be applied. Usually, generative tasks like text summarization or machine translation can be evaluated in this way. 

\textbf{\textit{Discriminative Tasks:}}
For tasks involving class prediction, post-processing using a parsing script is usually required to extract answers from the LLM-generated responses to compare against gold labels. In this context, metrics such as Exact Match, Accuracy, Precision, Recall, F1, are usually utilized in discriminative tasks \cite{laskar-etal-2023-systematic,qin2023chatgpt,bang2023multitaskchatgpt}. %LLM-generated responses often include extra information, such as descriptive explanations or synonyms for the class, beyond what is needed \cite{laskar-etal-2023-systematic}. 

\textbf{\textit{Generative Tasks:}} For generative tasks such as summarization or machine translation, parsing scripts are usually not required \cite{laskar-etal-2023-systematic,jahan2024comprehensive} and so the full response generated by LLMs are compared against the gold reference. In this regard, \textit{ROUGE} \cite{lin2004rouge} and \textit{BLEU} \cite{bleu} which are based on n-gram word matching are widely used. Meanwhile, various contextualized similarity-based metrics (e.g., \textit{BERTScore} \cite{zhang2019bertscore}) are also utilized that do not depend on word-based similarity measures.
% Responses might require post-processing for tasks that involve predicting a class to enable automatic evaluation metrics such as accuracy or F1 score. LLM generated responses often include extra information, such as descriptive explanations or synonyms for the class, beyond what is needed \cite{laskar-etal-2023-systematic}. Therefore, it is sometimes necessary to write parsing scripts to extract the target labels from these responses before calculating the evaluation metrics. While the created parsing scripts could be useful for many tasks, they may not necessarily be applicable to every discriminative task. For instance, \citet{jahan2024comprehensive} could not design any parsing scripts to accurately extract the relations between entities in LLM-generated responses and so they leveraged humans to evaluate the performance of LLMs in the relation extraction task. 
% For instance, in \textit{discriminative} tasks, usually parsing scripts are first utilized to extract the targeted answer from the LLM-generated response and then compared against the gold label. In this regard, \textit{exact match} accuracy is widely used to compare the answers extracted from the LLM-generated responses against the gold labels. In addition to \textit{exact match}, \textit{Precision}, \textit{Recall}, \textit{F1}, and \textit{Accuracy} are also used in discriminative tasks \cite{laskar-etal-2023-systematic,qin2023chatgpt,bang2023multitaskchatgpt}. 
 %   In this regard, \citet{laskar-etal-2023-systematic} investigated the performance difference in this regard. 
 %   \item \citet{jahan2024comprehensive} mentions that in relation extraction, it is a must to do human evaluation. 
% \end{enumerate}
%\end{itemize}
% based on \textit{fluency}, \textit{coherence}, \textit{informativeness}, and \textit{factual correctness} are also used \cite{fu2024tiny}. Since LLM-generated responses are usually descriptive, fluent, and also coherent, the hallucination problems \cite{huang2023survey} in LLMs make the qualitative evaluation of LLMs in terms of \textit{factual correctness} more important. 
\paragraph{Human Evaluation:}
Since LLMs generate human-like responses, it is often required to conduct qualitative evaluation of their responses. Recently, the Elo rating system \cite{zheng2024judging} that leverages humans to evaluate LLM-generated responses has gained a lot of attention. Other than that, the presence of hallucination \cite{rawte2023surveyhallucination,liu2023mitigatinghallucination} has made it more important to ensure trust and safety \cite{zhuo2023redteaming} in LLM-generated responses. In this regard, measuring factual correctness via humans has become more essential. %Below, we briefly describe the  Elo rating.


\paragraph{LLMs as Evaluators:}

% \begin{itemize}

Since human evaluation is time-consuming and difficult to reproduce, 
the instruction-following capabilities of LLMs have also inspired researchers to use certain LLMs-as-a-judge to evaluate the responses generated by other LLMs \cite{huang2024empirical}.  %For LLM-based evaluation, closed-source LLMs, especially the use of GPT-4 have become a standard practice in current studies. As discussed in Section \ref{}, due to the continuous updates of the closed-source LLMs, ensuring the reproducibility of this LLM-based evaluation could be an issue. To address this problem, more recently, the Prometheus-2 \cite{kim2024prometheus2} model has been proposed, which is an open-source LLM-based evaluator and demonstrates higher correlation with humans while outperforming various closed-source LLMs.


\fi
%\item \textbf{Are LLM as evaluators reliable? [Tahmid, Sawsan]: does it always collide with humans, identify limitations, can better prompt fix it? Check the MT bench and identify human correlation. }

%\textbf{Suggested resources (not limited to): }
%\begin{enumerate}
%    \item \url{https://arxiv.org/pdf/2404.18796}
 %   \item \url{https://arxiv.org/abs/2405.01724}
%      \item \url{https://arxiv.org/abs/2306.05685}
%\end{enumerate}
% \end{itemize}
%\end{enumerate}

%\subsection{Existing LLM Evaluation} 




%\item \textbf{RAG evaluation [Mizan, Tahmid]: What methodology is used for RAG evaluation and what are the existing limitations? Do we need human eval for RAG evaluation or can we rely on automatic metrics? Check: The Needle In a Haystack Test, Cohere. }
% https://twitter.com/emollick/status/1787472719065256092

%\textbf{Automatic Metrics}

%\textbf{Human Evaluation}

%\textbf{LLM as Evaluators}


%\end{itemize}



% \subsubsection{Evaluation Metrics} 
% \label{evaluation_metrics}

% The evaluation metrics for LLMs can be divided into two main categories: (i) those used for assessing language modeling performance ; (ii) those used for evaluating downstream task performance.

% %\begin{enumerate}[i.]
% \paragraph{Evaluating for Language Modeling:} Perplexity is widely used % evaluation metric 
%     to study the performance of auto-regressive language models. It measures how confidently a model predicts the next word in a sequence, with the assumption that lower perplexity indicates better performance. % Perplexity reflects the model's confidence in its predictions: lower perplexity signifies higher confidence. 
%     Hence, perplexity has been historically used to assess the language model's capability to generate a coherent language and is also useful to quickly compare different models or checkpoints.

% \paragraph{Evaluating on Downstream Tasks:} The evaluation metrics vary depending on the task. %\textit{evaluation metrics for discriminative tasks}, and (ii) \textit{evaluation metrics for generative tasks}. 
% For instance, in \textit{discriminative} tasks, usually parsing scripts are first utilized to extract the targeted answer from the LLM-generated response and then compared against the gold label. In this regard, \textit{exact match} accuracy is widely used to compare the answers extracted from the LLM-generated responses against the gold labels. In addition to \textit{exact match}, \textit{Precision}, \textit{Recall}, \textit{F1}, and \textit{Accuracy} are also used in discriminative tasks \cite{laskar-etal-2023-systematic,qin2023chatgpt,bang2023multitaskchatgpt}. Meanwhile, in \textit{generative} tasks, parsing scripts are usually not required \cite{laskar-etal-2023-systematic,jahan2024comprehensive} and so the full response generated by LLMs are compared against the gold reference. In this regard, \textit{ROUGE} \cite{lin2004rouge} and \textit{BLEU} \cite{bleu} which are based on n-gram word matching are widely used. Meanwhile, various contextualized similarity-based metrics (e.g., \textit{BERTScore} \cite{zhang2019bertscore}) are also utilized that do not depend on word-based similarity measures. In addition, qualitative evaluation based on \textit{fluency}, \textit{coherence}, \textit{informativeness}, and \textit{factual correctness} are also used \cite{fu2024tiny}. Since LLM-generated responses are usually descriptive, fluent, and also coherent, the hallucination problems \cite{huang2023survey} in LLMs make the qualitative evaluation of %\textit{informativeness} and 
% \textit{factual correctness} %via humans 
% more important. 
%\end{enumerate}


%\end{itemize}


%%The evaluation approach can be divided into the following: \textit{automatic evaluation}, \textit{human evaluation}, \textit{LLMs as evaluators}. In \textit{automatic evaluation}, often parsing scripts are utilized to extract the targeted answer, especially in discriminative tasks, followe metrics like Perplexity \cite{jelinek1977perplexity}, %Precision, Recall, F1, and Exact Match are directly utilized to compare the scores based on comparing the gold label with the generated answer. Since LLMs sometimes generate descriptive responses, often parsing scripts are utilized to extract the targeted answer, especially in discriminative tasks like classification \cite{laskar-etal-2023-systematic}. since LLMs generate human-like responses, it is often required to conduct qualitative evaluations of their responses to measure criteria like factual correctness, coherence, and informativeness. 
\if{false}
The evaluation approach can be divided into three categories: 

\begin{itemize}
    \item \textbf{Automatic Evaluation:} Where metrics like Perplexity \cite{jelinek1977perplexity}, Precision, Recall, F1, Exact Match, etc. are directly utilized to compare the scores based on comparing the gold label with the generated answer. Since LLMs sometimes generate descriptive responses, often parsing scripts are utilized to extract the targeted answer, especially in discriminative tasks like classification \cite{laskar-etal-2023-systematic}. 
   \item \textbf{Human Evaluation:} Since LLMs generate human-like responses, it is often required to conduct qualitative evaluations of their responses. This can be done to measure factual correctness, coherence, informativeness, etc. Moreover, the Elo rating system \cite{zheng2024judging} has gained a lot of attention for human evaluation. 

\item \textbf{LLMs as Evaluators:} Since human evaluation is time-consuming and difficult to reproduce, certain LLMs are used as a judge to evaluate the responses generated by other LLMs \cite{huang2024empirical}.

\end{itemize}

More details regarding the LLM evaluation approaches are discussed in Appendix \ref{appendix_evaluation_approach}.

\fi

%Ensuring reproducible results is a significant obstacle in the evaluation process. %\citet{biderman2024lessons} discuss the reproducibility issues in LLMs and have struggled to replicate the results reported in previous papers. When reproducibility during inference is lacking, results can vary across runs despite identical inputs and conditions.



% Aligned with the discussion in \cite{biderman2024lessons}, the inconsistency of results leads to several negative consequences, including unreliability, difficulty in comparing results across different setups, and reduced credibility. The most critical factor contributing to the difficulty in reproducing results is the lack of proper and comprehensive documentation for each part of the evaluation cycle. This includes details about the benchmarking datasets, prompt construction, the model being evaluated, decoding strategy, response parsing and cleaning processes, and the evaluation methodology.

% Thus, proper documentation of various details, such as the versions of the closed-source LLMs that have been used, as well as how the prompts were constructed, alongside analyzing the effects of prompt variations, should also be properly documented to ensure a fair reproduction of the results. 
% To address the reproducibility issue, \citet{kosch2024risk,mcintosh2024inadequacies} emphasize the importance of logging model versions, parameters, prompts, outputs, etc. to ensure the reproducibility of results. They highlight the issue of p-hacking, where developers selectively report statistical tests to achieve significant results, leading to false positives and compromised reproducibility, thus undermining scientific integrity. Below, we investigate various factors that may impact the reproducibility of existing evaluation of LLMs: % based on the following criteria: (i) Prompting, (ii) Parameter Settings, (iii) Updates in Model Versions. %[THE FOLLOWING IS MOVED TO THE END OF THE PROMPTING SECTION] Nonetheless, one major concern in this regard is prompt hacking, which involves manipulating input prompts to a language model to elicit desired responses, biasing the model's output, and compromising result integrity. Recognizing these parallels underscores the need for transparency and robust methodologies to maintain credibility in research and AI development.


% ,llm_eval_tist

%Evaluating LLM-generated responses is not a trivial task. Due to their ability to generate human-like responses, these models may sometimes produce unexpected responses which makes evaluation quite difficult. Therefore, it is sometimes necessary to write parsing scripts to extract the target labels from these responses before calculating the evaluation metrics %For this circumstance, it is often required to first design a parsing script to extract the desired answer from the LLM-generated response before applying task-specific evaluation criteria and metrics %are followed %in the existing literature 
%\cite{laskar-etal-2023-systematic,jahan2024comprehensive,llm_eval_tist}. %Effective parsing ensures that data extracted from model outputs is accurately aligned with evaluation criteria, thereby maintaining the accuracy and reliability of the assessments.

%While these parsing scripts can be useful for many tasks, they may not be applicable to every discriminative task. For instance, \citet{jahan2024comprehensive} could not design any parsing scripts to accurately extract relations between entities in LLM-generated responses, and thus, they leveraged human evaluators for assessing LLM performance in the relation extraction task.

%Below, we describe the design of parsing scripts to extract the targeted answers from LLM-generated responses, followed by discussing the prominent evaluation approaches: %, followed by the evaluation metrics: % we describe below: %Due to this difficulty and the need to effectively and efficiently evaluate the responses, different evaluation frameworks have been proposed as discussed below:
%it is often required to first design a parsing script to extract the desired answer from the LLM-generated response

% \subsubsection{Evaluation Approaches} 
% \label{evaluation_approach}

%LLM-generated responses may contain additional information than what is required \cite{laskar-etal-2023-systematic}, it is not trivial to evaluate LLMs in discriminative tasks. Therefore, task-specific parsing scripts are designed to extract the target labels from the LLM-generated responses.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Evaluating LLM-generated responses is not a trivial task. % since LLMs generate human-like responses instead of providing a probability distribution. 
%For instance, in discriminative tasks like text classification, instead of providing only the output class, they may also generate other descriptive texts or contain a synonym of the correct answer.  %(e.g., the class is X). 
%Meanwhile, LLMs may not consistently generate their responses in a specific format. For these reasons, some tasks are very challenging to evaluate based on directly comparing LLM-generated responses with the gold labels via %naive 
%string matching. To address these issues, task-specific evaluation methods are followed in the existing literature \cite{laskar-etal-2023-systematic,jahan2024comprehensive,llm_eval_tist} which we describe below:


% Since LLMs usually generate human-like responses instead of providing a probability distribution, it is not trivial to evaluate LLM-generated responses, especially in discriminative tasks, such as text classification. This is because in many cases, LLM-generated responses may contain descriptive text in addition to the answer, or they may contain a synonym of the gold answer. Meanwhile, LLMs may not be consistent in generating their responses in a specific format. For these reasons, some tasks are very challenging to evaluate based on just directly comparing LLM-generated responses with the gold labels based on naive string matching. To address these issues, task-specific evaluation methods are followed in the existing literature \cite{laskar-etal-2023-systematic,jahan2024comprehensive,llm_eval_tist} which we describe below:

%\begin{enumerate}[label=\roman*.]
%    \item \textbf{Automatic Evaluation:} Where they evaluate some tasks, such as text summarization via leveraging automatic evaluation scripts.
%    \item \textbf{Human Evaluation:} Where they evaluate some discriminative tasks solely by humans, which cannot be evaluated directly based on automatic evaluation scripts.
%    \item \textbf{Hybrid (Human + Automatic) Evaluation:} Where they evaluate some tasks via leveraging both human intervention alongside evaluation scripts. More specifically, this is done by first applying evaluation scripts on the dataset to parse the results from the LLM-generated response, followed by utilizing human intervention if solely depending on the evaluation script cannot parse the results in the expected format. 
%\end{enumerate}
%





%%%%%%%%%%%%%%%%%PARSING
%For example, when asked to generate only the class of a given input, the model might also include descriptive text or provide a synonym of the correct answer. Additionally, LLMs may not consistently format their responses in a specific manner. 
%For these reasons, some tasks are very challenging to evaluate based on directly comparing LLM-generated responses with the gold labels via %naive string matching. 


%some tasks are more difficult to evaluate as the results may not be directly comparable to the ground truth. 



%\begin{itemize}


%\item \textbf{Are parsing scripts good enough to extract the required LLM response or human evaluation is a must? Is Human Evaluation conducted in existing benchmarks or does the evaluation solely rely on parsing scripts [Tahmid, Mizan, Zarzis, Israt]}

%\textbf{Suggested resources (not limited to): }
%\begin{enumerate}
  %  \item 


% \paragraph{Evaluation Metrics} 
%\label{evaluation_metrics}

% The evaluation metrics for LLMs can be divided into two main categories: %(i) those used for assessing language modeling performance; (ii) those used for evaluating downstream task performance.

%\begin{enumerate}[i.]
